The Impact of Helium Exposure on the PMTs of the SuperNEMO Experiment

The performance of Hamamatsu 8" photomultiplier tubes (PMTs) of the type used in the SuperNEMO neutrinoless double-beta decay experiment (R5912-MOD), is investigated as a function of exposure to helium (He) gas. Two PMTs were monitored for over a year, one exposed to varying concentrations of He, and the other kept in standard atmospheric conditions as a control. Both PMTs were exposed to light signals generated by a Bi-207 radioactive source that provided consistent large input PMT signals similar to those that are typical of the SuperNEMO experiment. The energy resolution of PMT signals corresponding to 1 MeV energy scale determined from the Bi-207 decay spectrum, shows a negligible degradation with He exposure; however the rate of after-pulsing shows a clear increase with He exposure, which is modelled and compared to diffusion theory. A method for reconstructing the partial pressure of He within the PMT and a method for determining the He breakdown point, are introduced. The implications for long-term SuperNEMO operations are briefly discussed.

==> authors_2025_ageing.tex <==
\author[g c]{X.  Aguerre ,} 
\author[n]{R.  Arya ,} 
\author[q]{A.  Barabash ,} 
\author[h]{A.  Basharina-Freshville ,} 
\author[d]{M.  Bongrand ,} 
\author[i]{R.  Breier ,} 
\author[a]{J.  Busto ,} 
\author[c]{C.  Cerna ,} 
\author[h]{M.  Ceschia ,} 
\author[c]{E.  Chauveau ,} 
\author[f]{D.  Duchesneau ,} 
\author[n]{J.  Evans ,} 
\author[q]{D.  Filosofov ,} 
\author[d]{X.  Garrido,} 
\author[c]{M.  Granjon,} 
\author[d]{M.  Hoballah ,} 
\author[j]{R.  Hodak ,} 
\author[h]{R.  Horner,} 
\author[f]{A.  Jeremie ,} 
\author[i]{J.  Kaizer ,} 
\author[q]{A.  Klimenko ,} 
\author[q]{O.  Kochetov ,} 
\author[j r]{F.  Konarik ,} 
\author[q]{S.  Konovalov ,} 
\author[j r]{T.  Krizak ,} 
\author[c]{A.  Lahaie,} 
\author[b]{K.  Lang ,} 
\author[e]{Y.  Lemiere ,} 
\author[g]{E.  Li ,} 
\author[h]{A.  Liptak,} 
\author[j]{M.  Macko ,} 
\author[c]{C.  Marquet ,} 
\author[e]{F.  Mauger ,} 
\author[j s]{A.  Mendl ,} 
\author[p]{B.  Morgan ,} 
\author[q]{I.  Nemchenok ,} 
\author[j]{V.  Palusova ,} 
\author[n]{E.  Pape ,} 
\author[g]{C.  Patrick ,} 
\author[h]{T.  Pavicic,} 
\author[c]{F.  Perrot ,} 
\author[j]{M.  Petro ,} 
\author[i]{M.  Petro ,} 
\author[c]{F.  Piquemal ,} 
\author[i]{P.  Povinec ,} 
\author[g]{S.  Pratt ,} 
\author[b]{M.  Proga ,} 
\author[h]{W.  Quinn ,} 
\author[p]{Y.  Ramachers ,} 
\author[x]{C.  Riddle ,} 
\author[q]{N.  Rukhadze ,} 
\author[h]{R.  Saakyan ,} 
\author[b]{R.  Salazar ,} 
\author[d]{L.  Simard ,} 
\author[i]{F.  Simkovic ,} 
\author[k n]{S.  Soldner-Rembold ,} 
\author[j]{I.  Stekl ,} 
\author[o]{J.  Suhonen ,} 
\author[a]{H.  Tedjditi ,} 
\author[q]{V.  Timkin ,} 
\author[l m]{V.  Tretyak ,} 
\author[q]{V.  Tretyak ,} 
\author[g]{G.  Turnbull ,} 
\author[d]{Y.  Vereshchaka ,} 
\author[h]{D.  Waters ,} 
\author[q]{V.  Yumatov ,} 
\author[q]{A. Rahimov ,} 
\author[q]{A. Smolnikov ,} 

 
 
\affiliation[a]{Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France,}
\affiliation[b]{University of Texas at Austin Departement of Physics, Austin, TX 78712, USA,}
\affiliation[c]{Université de Bordeaux, CNRS/IN2P3, LP2i, Bordeaux, UMR 5797, F-33170, Gradignan, France,}
\affiliation[d]{Université Paris-Saclay, CNRS, IJCLab, F-91405, Orsay, France,}
\affiliation[e]{Université de Caen Normandie, ENSICAEN, CNRS/IN2P3, LPC Caen, UMR6534, F-14000, Caen, France,}
\affiliation[f]{LAPP, Université Savoie Mont Blanc, CNRS/IN2P3, Annecy, France,}
\affiliation[g]{University of Edinburgh, SUPA, School of Physics and Astronomy, Edinburgh, EH9 3FD, UK,}
\affiliation[h]{University College London, London, WC1E 6BT, UK,}
\affiliation[i]{Faculty of Mathematics Physics and Informatics, Comenius University, SK-842 48, Bratislava, Slovakia,}
\affiliation[j]{Institute of  Experimental and Applied Physics, Czech Technical University in Prague, CZ-11000 Prague, Czech Republic,}
\affiliation[k]{Imperial College London, London, SW7 2BZ, UK,}
\affiliation[l]{Institute for Nuclear Research of NASU, Kyiv, 03028, Ukraine,}
\affiliation[m]{INFN, Laboratori Nazionali del Gran Sasso, 67100, Assergi (AQ), Italy,}
\affiliation[n]{University of Manchester, Manchester, M13 9PL, UK,}
\affiliation[o]{Department of Physics, University of Jyväskylä, Jyvaskyla, Finland,}
\affiliation[p]{University of Warwick, Coventry, CV4 7AL, UK,}
\affiliation[q]{Participant in the NEMO-3/SuperNEMO collaboration}
\affiliation[r]{Faculty of Nuclear Sciences and Physical Engineering, Czech Technical University in Prague, Brehova, 7 115,  Czech Republic,}
\affiliation[s]{Faculty of Mathematics and Physics, Charles University, CZ-12116, Prague, Czech Republic,}

 
 
% Version 4 of paper authors

\author[a, l]{X.~Aguerre,}
\author[b]{A.S.~Barabash}
\author[c]{A.~Basharina-Freshville,}
\author[d]{M.~Bongrand,}
\author[d]{Ch.~Bourgeois,}

\author[d]{D.~Boursette,}
\author[d]{D.~Breton,}
\author[e]{R.~Breier,}
\author[f]{J.~Busto,}
\author[d]{S.~Calvez,}
\author[a]{C.~Cerna,}
\author[a]{E.~Chauveau,}
% \author[c]{A.~Chopra,}
% \author[c]{L.~Dawson,}

\author[g]{D.~Duchesneau,}
\author[h]{J.J.~Evans,}
\author[d]{X.~Garrido,}
\author[d]{C.~Girard-Carillo,}
\author[a]{M.~Granjon,}
\author[i]{B.~Guillon,}

\author[d]{M.~Hoballah,}
\author[j]{R.~Hodák,}
\author[c]{G.~Horner,}
% \author[a]{A.~Huber,}
% \author[c]{M.H.~Hussain,}
\author[c]{A.~Islam,}
\author[g]{A.~Jérémie,}
\author[d]{S.~Jullian,}
\author[b]{O.~Kochetov,}

\author[b]{S.I.~Konovalov,}
\author[b]{S.~Kovalenko,}
\author[a]{A.~Lahaie,}
\author[k]{K.~Lang,}
\author[i]{Y.~Lemière,}
\author[l]{P.~Li,}
%\author[k]{Z.~Liptak,}
\author[d]{P.~Loaiza,}

\author[d]{J.~Maalmi,}
\author[j]{M.~Macko,}
\author[j]{F.~Mamedov,}
\author[a]{C.~Marquet,}
\author[i]{F.~Mauger,}
\author[m]{B.~Morgan,}

\author[b]{I.~Nemchenok,}
\author[n]{M.~Nomachi,}
% \author[i]{G.~Oliviero,}
\author[j]{V.~Palusova,}
\author[l]{C.~Patrick,}
\author[c]{T.~Pavicic,}
\author[a]{F.~Perrot,}

\author[e,j]{M.~Petro,}
\author[a]{A.~Pin,}
\author[a]{F.~Piquemal,}
\author[e]{P.~Povinec,}
\author[l]{S.~Pratt,}
\author[k]{M.~Proga,}
\author[c]{W.S.~Quinn,}

\author[m]{Y.A.~Ramachers,}
% \author[g]{A.~Remoto,}
\author[o]{C.L.~Riddle,}
\author[c]{R.~Saakyan,}
\author[k]{R.~Salazar,}
\author[d]{X.~Sarazin,}
\author[p]{J.~Sedgbeer,}

\author[j]{Yu.~Shitov,}
\author[d]{L.~Simard,}
\author[e,j]{F.~Simkovic,}
\author[b]{A.~Smolnikov,}
\author[h,p]{S.~Söldner-Rembold,}
\author[j]{I.~Stekl,}

\author[q]{J.~Suhonen,}
\author[f]{H.~Tedjditi,}
\author[c]{J.~Thomas,}
\author[b]{V.~Timkin,}
\author[b]{V.I.~Tretyak,}
\author[r,s]{Vl.I.~Tretyak,}

\author[l]{G.~Turnbull,}
\author[b]{V.I.~Umatov,}
\author[d]{Y.~Vereshchaka,}
\author[c]{D.~Waters}
%\author[c]{and F.~Xie}

%------------------------------%

\affiliation[a]{Université de Bordeaux, CNRS/IN2P3, LP2i Bordeaux, UMR 5797, F-33170 Gradignan, France}
\affiliation[b]{Participant in the NEMO-3/SuperNEMO collaboration}
\affiliation[c]{University College London, London, WC1E 6BT, United Kingdom}
\affiliation[d]{Université Paris-Saclay, CNRS, IJCLab, F-91405 Orsay, France}
\affiliation[e]{Faculty of Mathematics, Physics and Informatics, Comenius University, SK-842 48 Bratislava, Slovakia}
\affiliation[f]{Aix-Marseille Université, CNRS, CPPM, F-13288 Marseille, France}
\affiliation[g]{Université de Savoie, CNRS/IN2P3, LAPP, UMR 5814, F-74941 Annecy-le-Vieux, France}
\affiliation[h]{University of Manchester, Manchester, M13 9PL, United Kingdom}
\affiliation[i]{Université de Caen Normandie, ENSICAEN, CNRS/IN2P3, LPC Caen UMR6534, F-14000 Caen, France}
\affiliation[j]{Institute of Experimental and Applied Physics, Czech Technical University in Prague, CZ-11000 Prague, Czech Republic}
\affiliation[k]{University of Texas at Austin, Austin, TX 78712, U.S.A.}
\affiliation[l]{University of Edinburgh, Edinburgh, EH9 3FD, United Kingdom}
\affiliation[m]{University of Warwick, Coventry, CV4 7AL, United Kingdom}
\affiliation[n]{Osaka University, 1-1 Machikaneyama Toyonaka, Osaka 560-0043, Japan}
\affiliation[o]{Idaho National Laboratory, Idaho Falls, ID 83415, U.S.A.}
\affiliation[p]{Imperial College London, London, SW7 2AZ, United Kingdom}
\affiliation[q]{Jyväskylä University, FIN-40351 Jyv¨askyl¨a, Finland}
\affiliation[r]{Institute for Nuclear Research of NASU, 03028 Kyiv, Ukraine}
\affiliation[s]{INFN - Laboratori Nazionali del Gran Sasso, 67100 Assergi (AQ), Italy}
